Pixel-based tracking detectors for a Low Q2 Tagger at EIC -- status report

The design of pixel-based tracking detectors for a Low Q2 Tagger in the Far Backward region of the ePIC detector at EIC is presented. The physics case is outlined, together with estimates of rates and resolutions, and the current design based on Timepix4 technology is introduced.

==> phyiscs.tex <==
\section{Physics case for a Low $Q^{2}$-tagger}
The EIC yellow report \cite{khalek2021science} gives many compelling physics cases that would require
a low $Q^{2}$-tagger. The primary detector will cover the range of $ -4<\eta<4$ for the measurement of electrons, photons, hadrons, and jets. To cover the kinematically important regions beyond that it requires auxiliary detectors in the far backward and forward regions. Unlike the primary detector 
these regions close to the beamline will have the added complications of high rates and backgrounds
and so any detector technologies used will have to be able to handle this.

The low $Q^{2}$-tagger will facilitate measurement of reactions with small cross sections where Q2 dependence is not critical. Here we can benefit from the large virtual photon flux for reactions such as : exclusive vector meson production in ep and eA, particularly for upsilon measurements at threshold; a meson spectroscopy programme, particularly with the charmonium-like sector
(XYZ); Time-like Compton scattering; and it will naturally extend the Q2 range of DIS processes.

For Time-like Compton scattering to fully detect the exclusive reaction, we need to detect 
the scattered lepton, recoil proton, and both decay leptons. The most interesting kinematics 
dependence is that of the invariant mass of the two leptons, which will be well reconstructed in 
the primary detector. Measuring the scatted electron will allow the s dependence to be measured as
well as giving some measure of the production four momentum transfer, or t. When coupled with proton 
detection in the far forward region there will be the possibility of applying exclusivity cuts.

For meson photoproduction the central detector acceptance is sufficient for all configurations to accept events from $Q^{2} > 0.1$ GeV$^{2}$ to large  $Q^{2}$. 
The lower limit on the scattered electron of $\eta>-3.5$ is restrictive for photoproduction events 
in the main detector, especially for higher collision energies. The photoproduction of 
Deeply Virtual Meson Production at higher energies will completely depend on
the low $Q^{2}$-tagger unless a significant enhancement of the backward region's electron 
acceptance is possible. More acceptance with a low $Q^{2}$-tagger would directly
translate into more measured photoproduction events. An increased acceptance would benefit $\Upsilon$ photoproduction near threshold, where the projected statistical precision is particularly low and the count rates would be dramatically improved in these regions.

The increased virtual photon flux from the tagger would allow a programme of meson spectroscopy to be
undertaken. Of great interest would be the possibility of photo-producing exotic charmonium-like mesons, so-called  XYZ states. Photoproduction is a particularly useful production mechanism as it is capable of, in-principle, generating all possible states with all spins and parities. 
It also removes difficulties in interpretation of peaks coming in fixed mass decays
as kinematic effects, such as triangle singularities, are largely removed. Observation of narrow peaks in invariant masses of final states such as $J/\psi$ and pions should provide conclusive proof of 
the existence of true resonant states.
The low $Q^{2}$-tagger would provide the s dependence of the reaction, and if the recoil
proton is detected in the far-forward detectors, provide exlusive final states. Measuring
the scattered electron would also allow an amplitude analysis of the reaction to be performed yielding
the quantum numbers of the states. This will be more powerful if the tagger resolution is 
sufficient to determine the scattering plane and angle, thereby giving the full polarisation state of
the virtual photon. 
